Order Doesn't Matter, But Reasoning Does: Training LLMs with Order-Centric Augmentation

Logical reasoning is essential for large language models (LLMs) to ensure accurate and coherent inference. However, LLMs struggle with reasoning order variations and fail to generalize across logically equivalent transformations. LLMs often rely on fixed sequential patterns rather than true logical understanding. To address this issue, we introduce an order-centric data augmentation framework based on commutativity in logical reasoning. We first randomly shuffle independent premises to introduce condition order augmentation. For reasoning steps, we construct a directed acyclic graph (DAG) to model dependencies between steps, which allows us to identify valid reorderings of steps while preserving logical correctness. By leveraging order-centric augmentations, models can develop a more flexible and generalized reasoning process. Finally, we conduct extensive experiments across multiple logical reasoning benchmarks, demonstrating that our method significantly enhances LLMs' reasoning performance and adaptability to diverse logical structures. We release our codes and augmented data in https://github.com/qianxiHe147/Order-Centric-Data-Augmentation.

==> 050answer.tex <==
\begin{table*}[t]
  \centering
  \scriptsize
  \renewcommand{\arraystretch}{1.5} % 增加行距
  \resizebox{0.7\textwidth}{!}{
\begin{tabular}{ll|cc|cc}
\hline
\multirow{\textbf{Models}} & \multirow{\textbf{Training data}} & \multicolumn{2}{c|}{\textbf{GSM8K}} & \multicolumn{2}{|c}{\textbf{FOLIO}}  \\ \cline{3-6} 
 &  & \textbf{Sequential} & \textbf{Shuffled} & \textbf{Sequential} & \textbf{Shuffled}  \\ \hline
\multirow{LLaMA2-13B-Chat} & Untrained &  &  &  & \\ 
 & Raw & 51.40\% & & 73.40\% & 70.69\%  \\  
 & + Condition Shuffling & \textbf{54.96\%} &  & \textbf{76.35\%} & \textbf{73.89\%} \\ \hline
\multirow{Mistral-7B-Instruct-v0.3} & Untrained &  &  &  &  \\  
 & Raw & & &67.47\% & 66.75\% \\  
 & + Condition Shuffling  & & & \textbf{72.91\%} &\textbf{72.17\%} \\ \hline
\end{tabular}
}
\caption{Model performance across datasets and answers}
\label{tab:model_performance}
\end{table*}



==> 050condition.tex <==
\begin{table*}[t]
  \centering
  \scriptsize
  \renewcommand{\arraystretch}{1.5} % 增加行距
  \resizebox{1\textwidth}{!}{
\begin{tabular}{ll|cc|cc|cc|cc}
\hline
\multirow{\textbf{Models}} & \multirow{\textbf{Training data}} & \multicolumn{2}{c|}{\textbf{GSM8K}} & \multicolumn{2}{|c|}{\textbf{FOLIO}} & \multicolumn{4}{|c}{\textbf{IFEVAL}} \\ \cline{3-10} 
 &  & \textbf{Sequential} & \textbf{Shuffled} & \textbf{Sequential} & \textbf{Shuffled} & \textbf{Sequential} & \textbf{Shuffled} & \textbf{Sequential} & \textbf{Shuffled} \\ \hline
\multirow{LLaMA2-13B-Chat} & Untrained &  &  &  &  & 32.00\% & 43.53\% & 14.10\% & 44.47\% \\ 
 & Raw & 47.30\% & & 69.95\% & 66.75\% & 49.91\% & 61.39\% & 26.92\% & 58.02\% \\  
 & + Condition Shuffling & \textbf{47.84\%} &  & \textbf{71.92\%} & \textbf{72.17\%} & \textbf{52.31\%} & \textbf{63.43\%} & \textbf{34.62\%} & \textbf{62.21\%} \\ \hline
\multirow{Mistral-7B-Instruct-v0.3} & Untrained &  &  &  &  &  &  & &  \\  
 & Raw & & &61.08\% & 59.36\% & 54.90\% & 66.43\% & 32.48\% & 61.07\% \\  
 & + Condition Shuffling  & & & \textbf{63.05\%} &\textbf{64.04\%} & \textbf{55.45\%} & \textbf{67.27\%} & \textbf{36.32\%} & \textbf{64.88\%} \\ \hline
\end{tabular}
}
\caption{Model performance across datasets and conditions}
\label{tab:model_performance}
\end{table*}



==> DAG_or_not_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\renewcommand{\arraystretch}{1.1} % 增加行间距到1.5倍
% 在表格环境之前设置全局字体为罗马字体
\renewcommand{\familydefault}{\rmdefault}
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccccc}
\toprule
\multirow{2}{*}{\textbf{Models}}            & \multirow{2}{*}{\textbf{Training data}} & \multicolumn{2}{c}{\textbf{FOLIO}} & \multicolumn{2}{c}{\textbf{Ruletaker}} & \multicolumn{2}{c}{\textbf{LogicNLI}} \\
\cmidrule(lr){3-8}
&                         & \textbf{Sequential}   & \textbf{Shuffled}   & \textbf{Sequential}     & \textbf{Shuffled}     & \textbf{Sequential}     & \textbf{Shuffled}    \\
\hline
\multirow{2}{*}{LLaMA3-8B-Instruct}
& Random Step Shuffled   & 76.85\%      & 69.21\%    & 82.10\% & 81.20\%      & \textbf{45.20\%} & 42.75\%     \\
& DAG-based Shuffled    & \textbf{77.34\%}      & \textbf{76.85\%}    & \textbf{84.60\%} & \textbf{82.70\%}      & 43.80\% & \textbf{42.80\%}     \\

\hdashline
\multirow{2}{*}{LLaMA2-13B-Chat}   
& Random Step Shuffled   & 71.92\%      & 69.21\%    & 74.75\% & \textbf{72.75\%}      & 43.70\% & 42.45\%     \\
& DAG-based Shuffled    & \textbf{76.35\%}      & \textbf{73.89\%}    & \textbf{75.50\%} & 72.25\%      & \textbf{46.90\%} & \textbf{42.75\%}     \\
\hdashline
\multirow{2}{*}{Mistral-7B-Instruct-v0.3} 
& Random Step Shuffled   & 71.43\%      & \textbf{72.41\%}    & 82.95\% & 79.95\%      & 44.75\% & 45.25\%    \\
& DAG-based Shuffled    & \textbf{72.91\%}      & 72.17\%    & \textbf{84.10\%} & \textbf{82.80\%}      & \textbf{47.35\%} & \textbf{47.30\%}     \\
\bottomrule
\end{tabular}
}
  \caption{
  The performance of the models using DAG-based step dependency for step reordering augmentation versus random step shuffling without dependencies.
  }
  \label{tab:DAG_or_not}
\end{table*}

==> main_result_new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% 提升用墨绿色
\begin{table*}[t]
% \newcolumntype{b}{>{\columncolor{blue!10}}c}
% \newcolumntype{d}{>{\columncolor{brown!10}}c}
\newcolumntype{g}{>{\columncolor{green!4}}c}
%\setlength\tabcolsep{7pt}
\newcolumntype{b}{>{\columncolor{blue!4}}c}
\renewcommand{\arraystretch}{1.2} % 增加行间距到1.5倍
% 在表格环境之前设置全局字体为罗马字体
\renewcommand{\familydefault}{\rmdefault}
\resizebox{\textwidth}{!}{
\begin{tabular}{llccccccgb}
\toprule
\multirow{2}{*}{\textbf{Models}}        & \multirow{2}{*}{\textbf{Training}} & \multicolumn{2}{c}{\textbf{FOLIO}}    & \multicolumn{2}{c}{\textbf{RuleTaker}}  & \multicolumn{2}{c}{\textbf{LogicNLI}}   & \multicolumn{2}{c}{\textbf{Avg.}} \\
\cmidrule(lr){3-10}
&             & \textbf{Seq.} & \textbf{Shf.} & \textbf{Seq.} & \textbf{Shf.} & \textbf{Seq.} & \textbf{Shf.} & \textbf{Seq.} & \textbf{Shf.} \\
\hline
\multirow{5}{*}{LLaMA3-8B-Instruct}     & Untrained   & 57.64\% & 55.17\% & 57.95\% & 57.95\% & 28.85\% & 25.50\% & -   & -           \\
& Vanilla SFT & 63.55\% & 61.82\% & 70.65\% & 68.65\% & 54.40\%  & 54.90\% & -   & -            \\
& + Condition Shuffled  & 70.44\%\textcolor{darkgreen}{(+6.89)} & 67.49\%\textcolor{darkgreen}{(+5.67)} & 81.70\%\textcolor{darkgreen}{(+11.05)} & 80.15\%\textcolor{darkgreen}{(+11.50)} & 59.95\%\textcolor{darkgreen}{(+5.55)} & 59.45\%\textcolor{darkgreen}{(+4.55)} & \textcolor{darkgreen}{(+7.83)}   & \textcolor{darkgreen}{(+7.24)}           \\
& SFT with COT  & 76.35\% & 73.65\% & 81.05\% & 78.80\% & 42.20\% & 41.65\% & -   & -  \\
& + Answer Steps Shuffled & 77.34\%\textcolor{darkgreen}{(+0.99)} & 76.85\%\textcolor{darkgreen}{(+3.20)} & 84.60\%\textcolor{darkgreen}{(+3.55)} & 82.70\%\textcolor{darkgreen}{(+3.90)} & 43.80\%\textcolor{darkgreen}{(+1.60)} & 42.80\%\textcolor{darkgreen}{(+1.15)} & \textcolor{darkgreen}{(+2.05)}   & \textcolor{darkgreen}{(+2.75)}           \\
& + Condition\&Answer Shuffled 
& 74.88\% (-2.46) 
& 75.86\% (-0.99) 
& 81.15\% (-3.45) 
& 79.60\% (-3.10) 
& 42.80\% (-1.00) 
& 43.50\% (+0.70) 
& (-2.30)   
& (-1.13) \\
\hdashline
\multirow{5}{*}{LLaMA2-13B-Chat}        & Untrained   & 39.16\% & 35.47\% & 53.30\% & 52.50\% & 28.45\% & 26.95\% & -   & -           \\
& Vanilla SFT & 53.69\% & 51.71\% & 65.35\% & 62.80\% & 45.65\% & 44.20\% & -   & -           \\
& + Condition Shuffled  & 63.05\%\textcolor{darkgreen}{(+9.36)} & 62.32\%\textcolor{darkgreen}{(+10.61)} & 72.20\%\textcolor{darkgreen}{(+6.85)} & 71.30\%\textcolor{darkgreen}{(+8.50)} & 54.00\%\textcolor{darkgreen}{(+8.35)} & 54.10\%\textcolor{darkgreen}{(+9.90)} & \textcolor{darkgreen}{(+8.19)}   & \textcolor{darkgreen}{(+9.67)}           \\
& SFT with COT  & 73.40\% & 70.69\% & 76.60\% & 74.65\% & 43.70\% & 39.30\% & -   & -           \\
& + Answer Steps Shuffled & 76.35\%\textcolor{darkgreen}{(+2.95)} & 73.89\%\textcolor{darkgreen}{(+3.20)} & 75.50\%\textcolor{red}{(-1.10)} & 72.25\%\textcolor{red}{(-2.40)} & 46.90\%\textcolor{darkgreen}{(+3.20)} & 42.75\%\textcolor{darkgreen}{(+3.45)} & \textcolor{darkgreen}{(+1.68)}   & \textcolor{darkgreen}{(+1.42)}         \\
& + Condition\&Answer Shuffled 
& 70.94\% (-5.41) 
& 67.24\% (-6.65) 
& 77.40\% (+1.90) 
& 73.80\% (+1.55) 
& 44.20\% (-2.70) 
& 41.60\% (-1.15) 
& (-2.07)   
& (-2.08) \\

% \hdashline
\cdashlinelr{1-10} 
\multirow{5}{*}{Mistral-7B-Instruct-v0.3} & Untrained   & 56.16\% & 57.39\% & 54.55\% & 54.55\% & 26.55\% & 24.90\% & -   & -           \\
& Vanilla SFT & 54.68\% & 55.17\% & 52.90\% & 53.20\% & 25.15\% & 25.05\% & -   & -           \\
& + Condition Shuffled  & 62.07\%\textcolor{darkgreen}{(+7.39)} & 61.82\%\textcolor{darkgreen}{(+6.65)} & 70.95\%\textcolor{darkgreen}{(+18.05)} & 69.20\%\textcolor{darkgreen}{(+16.00)} & 43.00\%\textcolor{darkgreen}{(+17.85)} & 44.20\%\textcolor{darkgreen}{(+19.15)} & \textcolor{darkgreen}{(+14.43)}   & \textcolor{darkgreen}{(+13.93)}          \\
& SFT with COT  & 67.47\% & 66.75\% & 81.55\% & 77.00\% & 46.40\% & 44.85\% & -   & -           \\
& + Answer Steps Shuffled & 72.91\%\textcolor{darkgreen}{(+5.44)} & 72.17\%\textcolor{darkgreen}{(+5.42)} & 84.10\%\textcolor{darkgreen}{(+2.55)} & 82.80\%\textcolor{darkgreen}{(+5.80)} & 47.35\%\textcolor{darkgreen}{(+0.95)} & 47.30\%\textcolor{darkgreen}{(+2.45)} & \textcolor{darkgreen}{(+2.98)}   & \textcolor{darkgreen}{(+4.56)}\\ 
& + Condition\&Answer Shuffled 
& 70.94\% (-1.97) 
& 70.44\% (-1.73) 
& 82.55\% (-1.55) 
& 81.70\% (-1.10) 
& 41.50\% (-5.85)
& 42.00\% (-5.30) 
& (-3.12)   
& (-2.71) \\

\bottomrule
\end{tabular}
}
  \caption{
  The overall performance on FOLIO, RuleTaker and LogicNLI.
  }
  \label{tab:main_result}
\end{table*}
